ExaGRyPE: Numerical General Relativity Solvers Based upon the Hyperbolic PDEs Solver Engine ExaHyPE

ExaGRyPE describes a suite of solvers for numerical relativity, based upon ExaHyPE 2, the second generation of our Exascale Hyperbolic PDE Engine. The presented generation of ExaGRyPE solves the Einstein equations in the CCZ4 formulation under a 3+1 foliation and focuses on black hole spacetimes. It employs a block-structured Cartesian grid carrying a higher-order order Finite Difference scheme with adaptive mesh refinement, it facilitates massive parallelism combining message passing, domain decomposition and task parallelism, and it supports the injection of particles into the grid as data probes or tracers. We introduce the ExaGRyPE-specific building blocks within ExaHyPE 2, and discuss its software architecture and compute-n-feel: For this, we formalize the creation of any specific simulation with ExaGRyPE as a sequence of lowering operations, where abstract logical tasks are successively broken into finer tasks until we obtain an abstraction level that can be mapped onto a C++ executable. The overall program logic is fully specified via a domain-specific Python interface, we map this logic onto a more detailed set of numerical tasks, subsequently lower this representation onto technical tasks that the underlying ExaHyPE engine uses to parallelize the application, before eventually the technical tasks are mapped onto task graphs including the actual PDE term evaluations, initial conditions, boundary conditions, and so forth. We end up with a rigorous separation of concerns which shields ExaGRyPE users from technical details and hence simplifies the development of novel physical models. We present the simulations and data for the gauge wave, static single black holes and rotating binary black hole systems, demonstrating that the code base is mature and usable. However, we also uncover domain-specific numerical challenges that need further study by the community in future work.

==> talks/pde-soft-abstract.tex <==

We present ExaHyPE 2 ("the Exascale Hyperbolic PDE solving Engine"), a powerful
tool for users to implement new hyperbolic PDEs solving applications. 
ExaHyPE 2 features a modular design, allowing users to easily construct their
simulation systems by only specifying the evolving quantities and terms of their PDEs. 
All technical complexities are handled by ExaHyPE 2 and its base mesh framework Peano 4. 
The latter provides adaptive grid management and mesh traversal support to the engine. 
The resulting application created by ExaHyPE 2 can be executed on various
platforms, from a student's laptop to state-of-the-art supercomputers, utilising
complete MPI+OpenMP parallelization. 
Additionally, ExaHyPE 2 offers extensive flexibility to advanced users, permitting them to modify nearly all code segments to suit the specific requirements of their simulations. In this talk, we will use our developing numerical relativity application as a case study to demonstrate the workflow of ExaHyPE 2, showcasing its strong capability in building new hyperbolic PDE-solving codes for complicated systems.


We present ExaHyPE 2, the second generation of the Exascale Hyperbolic PDE
Solver Engine.
It is a tool to implement solvers for hyperbolic PDEs given in first-order
formulation, while also providing support to second-order formulation via additional mesh sweep.
ExaHyPE 2 features a modular design, allowing users to easily compose their
simulation systems by only specifying the evolving quantities and terms of their PDEs. 
Once specified, ExaHyPE assembles the simulation code hiding parallelisation,
data structures, I/O, and so forth.
Based upon Peano 4, the code supports dynamically adaptive meshes.
The resulting application created by ExaHyPE 2 can be executed on various
platforms, ranging from laptops to supercomputers, with support for MPI, OpenMP,
TBB, and offloading to GPUs via OpenMP, C++ and SYCL.

In this talk, we will use our numerical relativity application as
case study to demonstrate the workflow behind ExaHyPE 2, which is now completely
Python-based, as opposed to a mixture of C++ and parameter files in ExaHyPE 1.
We also showcase which ingredients (such as numerical schemes) had to be changed
due to the application, and how ExaHyPE 2 supports this via the composition of
various solvers and their tailoring. 

% ExaHyPE 2: An Engine for Hyperbolic PDEs Solving Codes—Numerical Relativity Application as a Case Study.
%We present ExaHyPE 2, the second generation of the Exascale Hyperbolic PDE Solver Engine. It is a tool to implement solvers for hyperbolic PDEs given in first-order formulation, while also providing support to second-order formulation via additional mesh sweep. ExaHyPE 2 features a modular design, allowing users to easily compose their simulation systems by only specifying the evolving quantities and terms of their PDEs. Once specified, ExaHyPE assembles the simulation code hiding parallelisation, data structures, I/O, and so forth. Based upon Peano 4, the code supports dynamically adaptive meshes. The resulting application created by ExaHyPE 2 can be executed on various platforms, ranging from laptops to supercomputers, with support for MPI, OpenMP, TBB, and offloading to GPUs via OpenMP, C++ and SYCL.

%In this talk, we will use our numerical relativity application as case study to demonstrate the workflow behind ExaHyPE 2, which is now completely Python-based, as opposed to a mixture of C++ and parameter files in ExaHyPE 1. We also showcase which ingredients (such as numerical schemes) had to be changed due to the application, and how ExaHyPE 2 supports this via the composition of various solvers and their tailoring. 

% ExaHyPE 2: An Engine for Hyperbolic PDEs Solving Codes— ExaGRyPE as a Case Study.
%We present ExaHyPE 2, the second generation of the Exascale Hyperbolic PDE Solver Engine. It is a tool to implement solvers for hyperbolic PDEs given in first-order formulation, while also providing support to second-order formulation via additional mesh sweep. ExaHyPE 2 features a modular design, allowing users to easily compose their simulation systems by only specifying the evolving quantities and terms of their PDEs. Once specified, ExaHyPE assembles the simulation code hiding parallelisation, data structures, I/O, and so forth. Based upon Peano 4, the code supports dynamically adaptive meshes. The resulting application created by ExaHyPE 2 can be executed on various platforms, ranging from laptops to supercomputers, with support for MPI, OpenMP, TBB, and offloading to GPUs via OpenMP, C++ and SYCL.

%In this talk, we will introduce our numerical relativity code ExaGRyPE, and use it as a case study to demonstrate the workflow behind ExaHyPE 2. We also showcase which ingredients (such as numerical schemes) had to be changed due to the application, and how ExaHyPE 2 supports this via the composition of various solvers and their tailoring. 
